Background Subtraction via Fast Robust Matrix Completion

Background subtraction is the primary task of the majority of video inspection systems. The most important part of the background subtraction which is common among different algorithms is background modeling. In this regard, our paper addresses the problem of background modeling in a computationally efficient way, which is important for current eruption of "big data" processing coming from high resolution multi-channel videos. Our model is based on the assumption that background in natural images lies on a low-dimensional subspace. We formulated and solved this problem in a low-rank matrix completion framework. In modeling the background, we benefited from the in-face extended Frank-Wolfe algorithm for solving a defined convex optimization problem. We evaluated our fast robust matrix completion (fRMC) method on both background models challenge (BMC) and Stuttgart artificial background subtraction (SABS) datasets. The results were compared with the robust principle component analysis (RPCA) and low-rank robust matrix completion (RMC) methods, both solved by inexact augmented Lagrangian multiplier (IALM). The results showed faster computation, at least twice as when IALM solver is used, while having a comparable accuracy even better in some challenges, in subtracting the backgrounds in order to detect moving objects in the scene.

==> P_Rezaei_BackgroundSub_RSL-CV 2017/figs.tex <==
\newcommand{\figbs}{
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth,  trim=0in 0.1in 0in 0.1in,
  clip=true]{images/BS.jpg}
 % \vspace{-.15in}
  \caption{Standard structure common in the majority of the robust background subtraction methods.}
\label{fig:bs}
\vspace{-.2in}
\end{figure}
}
\newcommand{\figrpca}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.7\textwidth,  trim=2.3in 0.2in 2.3in 0.65in,
  clip=true]{images/rpca_video003_thresholded.eps}
  \vspace{-.2in}
  \caption{Results of applying RPCA on the BMC wandering students video demonstrated for 4 different frames; first row is the original frame, second row is the binary mask of the foreground by thresholding the detected foreground, and last row is the background image.}
\label{fig:rpca}
\vspace{-.1in}
\end{figure*}
}

\newcommand{\figmcv}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.7\textwidth,  trim=2.3in 0.2in 2.3in 0.4in,
  clip=true]{images/mc_v1_video003_bw.eps}
  \vspace{-.2in}
  \caption{Results of applying our fRMC on the BMC wandering students video for 4 different frames; first row is the original frame, second row is the binary mask of the foreground, and last row is the background image.}
\label{fig:mcv}
\vspace{-.1in}
\end{figure*}

}

\newcommand{\figbmc}{
\begin{figure*}[t]
 \centering
 \subfloat[]{\label{fig:rpca}\includegraphics[width=0.33\textwidth, trim=3in 0in 3in 0in,
  clip=true]{images/RPCA_BMCvid003_0223_0384.png}}
 \subfloat[]{\label{fig:rmc}\includegraphics[width=0.33\textwidth,trim=3in 0in 3in 0.25in,
  clip=true]{images/RMC_BMCvid003_0223_0384.png}}
  \subfloat[]{\label{fig:frmc}\includegraphics[width=0.33\textwidth,  trim=3in 0in 3in 0in,
  clip=true]{images/fRMC_BMCvid003_0223_0384.png}} 
  \caption{Result of applying the three methods (a) RPCA, (b) RMC, and (c) fRMC on BMC wandering students video demonstrated for two different frames; first row is the original frame, second row is the binary mask of the foreground by thresholding the detected foreground, and last row is the background image.}
\label{fig:bmc}
\vspace{-.2in}
\end{figure*}
}

\newcommand{\figsabs}{
\begin{figure*}[t]
 \centering
 \subfloat[]{\label{fig:rpca}\includegraphics[width=0.33\textwidth, trim=3in 0in 3in 0in,
  clip=true]{images/RPCA_SABSlightswitch_0302_-0440.png}}
 \subfloat[]{\label{fig:rmc}\includegraphics[width=0.33\textwidth,trim=3in 0in 3in 0.25in,
  clip=true]{images/RMC_SABSlightswitch_0302_-0440.png}}
  \subfloat[]{\label{fig:frmc}\includegraphics[width=0.33\textwidth,  trim=3in 0in 3in 0in,
  clip=true]{images/fRMC_SABSlightswitch_0302_-0440.png}} 
  \caption{Result of applying the three methods (a) RPCA, (b) RMC, and (c) fRMC on SABS light switch video demonstrated for two different frames; first row is the original frame, second row is the binary mask of the foreground by thresholding the detected foreground, and last row is the background image. As you can see RMC fails in modeling the background in abrupt change of light.}
\label{fig:sabs}
\vspace{-.1in}
\end{figure*}
}

==> P_Rezaei_BackgroundSub_RSL-CV 2017/tabs.tex <==
\newcommand{\tablresultBMC}{
\begin{table*}[]  
\small
\begin{center}  
\caption{Computational time and benchmark metrics for the background subtraction task of our fRMC algorithm compared to RPCA and RMC evaluated on the BMC dataset.}
 \begin{tabular}{| c | c | c | c | c | c | c |} 
 \hline
   Algorithm & Running time (min) & F-measure & D-score & Precision & PSNR & Ssim \\ 
 \hline
  \rowcolor[gray]{0.8}
 \multicolumn{7}{|c|} {Big trucks}  \\
 \hline
 RPCA        &  18           & 0.68  & 0.010 & 0.80 & 26.98 & 0.92 \\ 
 \hline
 RMC         &  29.6         & 0.76   & 0.0088  & 0.93 & 29.0 & 0.93  \\ 
 \hline
\text{fRMC}  &  \textbf{8.4} & \textbf{0.79} & \textbf{0.0087} & \textbf{0.94} & \textbf{30.07} & \textbf{0.94} \\ 
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{7}{|c|}{Wandering students} \\
 \hline
 RPCA  &  6.2 & 0.87 & 0.0062 & 0.90 & 46.03 & 0.97 \\
 \hline
 RMC &  12 & 0.80  & 0.0094 & \textbf{0.94}  & 42.93 & 0.97 \\ 
 \hline
 \text{fRMC}  &  \textbf{3.4} & \textbf{0.87} & \textbf{0.0061} & 0.90 & \textbf{46.11} & 0.97 \\
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{7}{|c|}{Rabbit in the night} \\
 \hline
 RPCA &  28 & 0.60 & 0.0053 & 0.61 & 41.19 & 0.97 \\ 
 \hline
 RMC &  30.3 & \textbf{0.76}  & \textbf{0.0035} & \textbf{0.91}  & \textbf{48.04}  & 0.98 \\ 
 \hline
 \text{fRMC}  &  \textbf{8.6} & 0.75 & 0.0037 & 0.85 & 47.42 & \textbf{0.99} \\
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{7}{|c|}{Beware of the trains} \\
 \hline
 RPCA  & 11.46 & 0.683 & 0.105 & 0.778 & 33.348 & 0.95 \\
 \hline
 RMC &  16 & 0.64  & 0.0091 & 0.83 & 32.94 & 0.95 \\ 
 \hline
 \text{fRMC} & \textbf{4.3} & \textbf{0.71} & \textbf{0.0084} & \textbf{0.89} & \textbf{34.3} & \textbf{0.96} \\
\hline
  \rowcolor[gray]{0.8}
\multicolumn{7}{|c|}{Train in the tunnel} \\
 \hline
 RPCA  & 14.2 & 0.63 & \textbf{0.0076} & 0.81 & 27.18  & 0.93  \\
 \hline
 RMC &  26.8 & \textbf{0.78}  & 0.0085  & 0.90 & \textbf{30.59} & \textbf{0.94} \\ 
 \hline
 \text{fRMC}  & \textbf{7.8} & \textbf{0.78}  & 0.0086 & \textbf{0.91} & \textbf{30.59} & \textbf{0.94} \\
\hline

\end{tabular}
\label{tbl:BMCresults}
\end{center}
\vspace{-.2in}
\end{table*}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tablresultSABS}{
\begin{table}[]  
\small
\begin{center}  
\caption{Computational time and benchmark metrics for the background subtraction task of our fRMC algorithm compared to RPCA and RMC evaluated on the SABS datasets.$^\star$shows the best result for each experiment reported by VIS for SABS dataset.}
 \begin{tabular}{| c | c | c | c |} 
 \hline
   Algorithm & Running time (min) & Precision & F-measure  \\ 
 \hline
  \rowcolor[gray]{0.8}
 \multicolumn{4}{|c|} {Basic}  \\
 \hline
 RPCA & 9.2  & \textbf{0.734}  &  0.775   \\ 
 \hline
 RMC & 45.0   & 0.732   & 0.778  \\ 
 \hline
\text{fRMC}  &  \textbf{6.2} &  0.732  & 0.779 \\ 
 \hline
 Best result$^\star$ & - & - & \textbf{0.800} \\
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{4}{|c|}{Light switch} \\
 \hline
 RPCA  & 9.0  & \textbf{0.725} & 0.506  \\
 \hline
 RMC & 44.0  & 0.100  & 0.163  \\ 
 \hline
 \text{fRMC}  & \textbf{6.3}  & 0.705 & \textbf{0.495}  \\
 \hline
 Best result & - & - & 0.316 \\
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{4}{|c|}{Camouflage} \\
 \hline
 RPCA & 8.8  & 0.742 & 0.747 \\ 
 \hline
 RMC & 45  & 0.746  & 0.752  \\ 
 \hline
 \text{fRMC}  & \textbf{5.6}   & \textbf{0.746} & 0.753  \\
 \hline
 Best result & - & - & \textbf{0.820} \\
 \hline
   \rowcolor[gray]{0.8}
 \multicolumn{4}{|c|}{No camouflage} \\
 \hline
 RPCA  & 9.6 & \textbf{0.752} & 0.7649 \\
 \hline
 RMC & 44.3  &  0.751 & 0.769  \\ 
 \hline
 \text{fRMC} & \textbf{6.0}  & 0.750  & 0.769   \\
\hline
Best result & - & - & \textbf{0.829} \\
 \hline
  \rowcolor[gray]{0.8}
\multicolumn{4}{|c|}{Noisy night} \\
 \hline
 RPCA  & 9.0  & \textbf{0.889} & 0.539  \\
 \hline
 RMC & 44.2  & 0.725  & 0.527  \\ 
 \hline
 \text{fRMC}  & \textbf{5.1}  & 0.726 & \textbf{0.528} \\
\hline
Best result & - & - & 0.321 \\
 \hline
 \rowcolor[gray]{0.8}
\multicolumn{4}{|c|}{MPEG4 (40Kbps)} \\
 \hline
 RPCA  & 9.5 & 0.662 & \textbf{0.779}   \\
 \hline
 RMC & 44.6  & \textbf{0.715} & 0.777  \\ 
 \hline
 \text{fRMC}  & \textbf{5.4}  & \textbf{0.714}   & 0.776 \\
\hline
Best result & - & - & 0.774 \\
 \hline

\end{tabular}
\label{tbl:SABSresults}
\end{center}
\vspace{-.2in}
\end{table}
}

